Application of DInSAR Technique to High Coherence Satellite Images for Strategic Infrastructure Monitoring

In this paper the authors present and validate a procedure, which intends to combine the latest state of the art models in bridge monitoring with freely available satellite data. Through the Differential SAR interferometry (DinSAR) technique, a dataset of displacements for the Morandi bridge in Genoa (Italy), before its collapse, has been created, by using images downloaded by the Copernicus Open-Access Hub and the ASFVertex Hub. The data have been processed through the ESA SNAP software to identify the rate of displacements in the parts of the bridge where collapse occurred. Results demonstrate that the adopted procedure has great potentiality in the application field, as it represents a simple and inexpensive method to monitor large structures in a continuous way, by helping to better quantify risks and guide effective mitigation countermeasures. Moreover, the same procedure, once properly validated, could be effectively extended to the current and future performance estimation of civil infrastructures.

==> Paper Ponte Morandi/old_itro.tex <==
\section{Introduction}
\label{sec:intro}
Nowadays  the combined use of remote sensing data and in situ data has allowed to improve the Earth Observation techniques allowing the validation of the results from the processing of satellite images such as those of Sentinel-1 and Sentinel-2 (us and Sica ), 

with the ability to monitor the Earth's surface and proceed with the classification of phenomena related to Geohazard Assessment, such as landslides for instance, but not only to them.
Data combination at this aim has been found very recently great attention and it has shown to increase robustness of results analysis.
In addition, very advanced techniques, such as Machine Learning and deep Learning, are progressively arising the interest of researchers in helping EO analysis for classification and detection.
Actually, very few papers present work and results in terms of detection, while something more has been published in terms of classification. 
In this paper authors aim to present their work, born on a collaboration between University of Sannio and MIT MISTI Italy, that has allowed to take different contribution and expertise to analyze the problem.
Main focus among critical geotechnical phenomena has been given to landslides, by starting to identify the five biggest landslides occurred between year x and year y.
The on line world database xxcddd has been used.  Satellite data used to feed the Machine Learning and Deep Learning algorithms have been remote sensing images from Copernicus Sentinel-1 and Sentinel-2 .
It has been thought to look for and download also data on rainfalls for the regions under analysis, to see if a correlation can be found between these phenomena and landslides, in particular.
Once the algorithms have been educated, known Case Studies will be used to check and validate the results and understand if these algorithms well perform in identifying the features that should anticipate the critical phenomena (forecasting them). 

Necessary some  references to show how the state of the art highlights the usefulness of using Sentinel data for the Geohazard assessment not only in the case of landslides but also in other geological and geotechnical phenomena (flood consequences, hydrogeologic changes and their impact, etc.).
United to in situ data for validation. Here I can also refer to a landslide situation near the dams for ex. (dams in the ground, ... I ask Stefania better), where the data collected by the instruments positioned on the dams (piezometers, axes, etc.) can serve to gather useful information on any movements detected in areas near the dam under analysis through the images satellite, and induced by land changes, landslides, also induced (but not only) by hydrogeological changes, etc. (Other  references are necessary).
Much more recently to these techniques and to this type of data combination (remote sensing and in situ), we have added the use of machine learning and deep learning algorithms (and here I put all the references we found), I mean that is at the beginning and only a few really say they do it and then they really do it.
We need  to highlight the major difficulties: processing big amount of data, which in the case of satellite imagery means first of all once identified, download images, store them, pre-process them (see problems related to georeferencing, when necessary, cloud masking, when necessary ... Sentinel-1 ... Sentinel-2 ... respectively).
A solution, perhaps, cloud services and computing services distributed online .... we do not know ... to check.
What do I need from you, in Italian, a summary of all the information to be added, considering that if the abstract is accepted it seems to me that there are several months to send the final paper (April or May and 'on the site).
The idea: to identify 5 large landslides (all the data, areas, coordinates, which site you used to find them, how, etc.), how we are proceeding images before and after Sentinel-1 and Sentinel-2, for now let's put it this way, explain to me better the problems / difficulties we are facing, data no longer available before ...., time to download those available, for Sentinel-1, presence of clouds for Sentinel-2, etc. etc.

==> old_itro.tex <==
\section{Introduction}
\label{sec:intro}
Nowadays  the combined use of remote sensing data and in situ data has allowed to improve the Earth Observation techniques allowing the validation of the results from the processing of satellite images such as those of Sentinel-1 and Sentinel-2 (us and Sica ), 

with the ability to monitor the Earth's surface and proceed with the classification of phenomena related to Geohazard Assessment, such as landslides for instance, but not only to them.
Data combination at this aim has been found very recently great attention and it has shown to increase robustness of results analysis.
In addition, very advanced techniques, such as Machine Learning and deep Learning, are progressively arising the interest of researchers in helping EO analysis for classification and detection.
Actually, very few papers present work and results in terms of detection, while something more has been published in terms of classification. 
In this paper authors aim to present their work, born on a collaboration between University of Sannio and MIT MISTI Italy, that has allowed to take different contribution and expertise to analyze the problem.
Main focus among critical geotechnical phenomena has been given to landslides, by starting to identify the five biggest landslides occurred between year x and year y.
The on line world database xxcddd has been used.  Satellite data used to feed the Machine Learning and Deep Learning algorithms have been remote sensing images from Copernicus Sentinel-1 and Sentinel-2 .
It has been thought to look for and download also data on rainfalls for the regions under analysis, to see if a correlation can be found between these phenomena and landslides, in particular.
Once the algorithms have been educated, known Case Studies will be used to check and validate the results and understand if these algorithms well perform in identifying the features that should anticipate the critical phenomena (forecasting them). 

Necessary some  references to show how the state of the art highlights the usefulness of using Sentinel data for the Geohazard assessment not only in the case of landslides but also in other geological and geotechnical phenomena (flood consequences, hydrogeologic changes and their impact, etc.).
United to in situ data for validation. Here I can also refer to a landslide situation near the dams for ex. (dams in the ground, ... I ask Stefania better), where the data collected by the instruments positioned on the dams (piezometers, axes, etc.) can serve to gather useful information on any movements detected in areas near the dam under analysis through the images satellite, and induced by land changes, landslides, also induced (but not only) by hydrogeological changes, etc. (Other  references are necessary).
Much more recently to these techniques and to this type of data combination (remote sensing and in situ), we have added the use of machine learning and deep learning algorithms (and here I put all the references we found), I mean that is at the beginning and only a few really say they do it and then they really do it.
We need  to highlight the major difficulties: processing big amount of data, which in the case of satellite imagery means first of all once identified, download images, store them, pre-process them (see problems related to georeferencing, when necessary, cloud masking, when necessary ... Sentinel-1 ... Sentinel-2 ... respectively).
A solution, perhaps, cloud services and computing services distributed online .... we do not know ... to check.
What do I need from you, in Italian, a summary of all the information to be added, considering that if the abstract is accepted it seems to me that there are several months to send the final paper (April or May and 'on the site).
The idea: to identify 5 large landslides (all the data, areas, coordinates, which site you used to find them, how, etc.), how we are proceeding images before and after Sentinel-1 and Sentinel-2, for now let's put it this way, explain to me better the problems / difficulties we are facing, data no longer available before ...., time to download those available, for Sentinel-1, presence of clouds for Sentinel-2, etc. etc.
